Scenario-Based Proofs for Concurrent Objects [Extended Version]

Concurrent objects form the foundation of many applications that exploit multicore architectures and their importance has lead to informal correctness arguments, as well as formal proof systems. Correctness arguments (as found in the distributed computing literature) give intuitive descriptions of a few canonical executions or "scenarios" often each with only a few threads, yet it remains unknown as to whether these intuitive arguments have a formal grounding and extend to arbitrary interleavings over unboundedly many threads. We present a novel proof technique for concurrent objects, based around identifying a small set of scenarios (representative, canonical interleavings), formalized as the commutativity quotient of a concurrent object. We next give an expression language for defining abstractions of the quotient in the form of regular or context-free languages that enable simple proofs of linearizability. These quotient expressions organize unbounded interleavings into a form more amenable to reasoning and make explicit the relationship between implementation-level contention/interference and ADT-level transitions. We evaluate our work on numerous non-trivial concurrent objects from the literature (including the Michael-Scott queue, Elimination stack, SLS reservation queue, RDCSS and Herlihy-Wing queue). We show that quotients capture the diverse features/complexities of these algorithms, can be used even when linearization points are not straight-forward, correspond to original authors' correctness arguments, and provide some new scenario-based arguments. Finally, we show that discovery of some object's quotients reduces to two-thread reasoning and give an implementation that can derive candidate quotients expressions from source code.

==> alg.tex <==
\section{Algorithm to compute a layer automaton for an SWO}
\label{apx:alg}

\SetKwFunction{kwWP}{WP}
\SetKwFunction{kwSP}{SP}
\SetKwFunction{kwAtomicPreds}{AtomicPredicates}
\SetKw{kwLet}{let}
\SetKw{kwIn}{in}
\begin{algorithm}[t]
\KwIn{An SWO object $O$}
\KwResult{Layer automaton $\mathcal{A}$}

\Begin{
%\tcp{Uses WPs of write operations to determine predicates to distinguish ADT states}
%$\bar{\varphi}_{pre}$ := $\emptyset$\;
\ForEach{$k\in\supp(\lyr)$ with $\lyr\in \Lyrs(O)$}{
   $Pre(k) =$  \kwWP($k,\mathit{true}$)
}
%\kwLet $[p_1,\ldots,p_n]$ = \kwAtomicPreds($\{Pre(\lyr): \lyr\in \Lyrs(O)\}$) \kwIn\;
\kwLet $\QQ=\{l_1\land\ldots\land l_n: \forall i\in [1,n].\ \exists k.\ Pre(k)\neq \mathit{false}\mbox{ and }l_i = Pre(k) \mbox{ or }l_i = \neg Pre(k)\}$ \kwIn\;
\kwLet $\QQ_0=\{q\in \QQ: \exists\env.\ C_0^\env\models q\}$ \kwIn\;
\ForEach{(local or write) layer $\lyr\in \Lyrs(O)$}{
   \ForEach{ $\qq{} \in \QQ{}$}{ 
   	\If{$\qq{} \Rightarrow \bigwedge_{k\in\supp(\lyr)} Pre(k)$} {
		\If{$\lyr$ is a local layer}{
			$\trans \stackrel{\cup}{=} \qq{} \xrightarrow{\lyr}\qq{}$\; 
		}
		\Else{
%			$Post(\qq{},\lyr) = $ \kwSP($\qq{},\supp(\lyr)$)\;
			\ForEach{ $\qq{}' \in \QQ{}$}{ 
%				\ForEach{ $k\in\supp(\lyr)$}{ 
				\If{for each $k\in\supp(\lyr)$, $[q]\cdot k\cdot \texttt{assert}\ \neg q'$ violates the assertion} { %\kwSP$(\qq{},\supp(\lyr)) \land \qq{}'$ satisfiable
					$\trans \stackrel{\cup}{=} \qq{} \xrightarrow{\lyr}\qq{}'$\; 
				}
%				}
			}
		}
   	}
   }
}
\Return{$\mathcal{A}=\langle \QQ{}, \QQ_0, \Lyrs(O),\delta \rangle$}\;
}
\caption{\label{alg:alg} Constructing a layers automaton.}
\end{algorithm}


Algorithm~\ref{alg:alg} describes a procedure for computing a layer automaton for an SWO object. This procedure starts by constructing the set of states, which represent boolean conjunctions of non-false weakest pre-conditions\footnote{The pre-conditions constrain the shared state and the arguments of the invocations that contain the paths in the support of a layer, and can include existential quantifiers (see Section~\ref{ssec:listset}).} of expressions\footnote{Recall that for an expression $\kat_l^1\kdot\kat_w\kdot \kat_l^2$ in the support of a write layer, we assume that the two paths $\kat_l^1\kdot \kat_l^2$ and $\kat_w$ are executed by different threads and therefore, local variables are renamed to be distinct.} in the \emph{support} of a layer of $O$ (assuming the post-condition $\mathit{true}$), or negations thereof. 
%When computing weakest pre-conditions of a write layer support $\kat_l^1\kdot \kat_w\kdot \kat_l^2$, we implicitly assume that the two paths $\kat_l^1\kdot \kat_l^2$ and $\kat_w$ are executed by different threads and therefore, local variables used in the two paths are renamed to avoid collisions. 
Interestingly, reasoning about supports of layers instead of ``full'' layers (recall that the support concretizes the Kleene star in a layer to a single repetition) is sound because the omitted actions are local and they can be ``replicated'' without affecting the feasibility of a trace. The set of initial states is defined as the set of states that are satisfied by some initial configuration (w.r.t. some environment $\env$).
Then, for each layer which is enabled in a given state $q$, \ie~$q$ implies the pre-condition of its support, it adds transitions starting in $q$ and labeled with that layer. For local layers, it adds a single transition that ends in the same state (because they contain only local actions that do not interfere with other threads), while for write layers, it adds a transition to every state $q'$ that can hold after executing that write layer. The latter is encoded as an assertion violation in a program that assumes that $q$ holds initially, executes any expression in the support of the layer (renaming local variables in different paths as for weakest pre-conditions), and asserts the negation of $q'$.

\begin{example}
Applying Algorithm~\ref{alg:alg} to $O_{ctr}$ begins with enumerating the support $\supp(\lambda)$ of each layer and computing the weakest precondition. In most cases the weakest precondition is simply \emph{true} and, in one case (namely, $\lambda_{dec0}$ which involves paths where decrement returns 0), the precondition is the test $[\code{ctr=0}]$. We thus define 
$\QQ=\{[\code{ctr=0}],\overline{[\code{ctr=0}]}\}$ based on this test and its negation.

The algorithm proceeds to enumerate local and write layers along with pre/post states. Consider 
$\qq=[\code{ctr=0}]$ and $\qq'=\overline{[\code{ctr=0}]}$ and $\lambda_{inc}$, with $\supp(\lambda_{inc})$ given in Example~\ref{ex:support}. One KAT expression $k\in\supp(\lambda_{inc})$ is: $k=[\ttc_r\code{:=ctr}] \kdot \kat_{inc} \kdot \overline{[\ttc_r\code{=ctr}]}$.
For this $k$, a solver can prove that
$[q]\cdot k\cdot \texttt{assert}\ \neg q'$ violates the assertion. Our algorithm therefore augments $\delta$ with  triple
$
\qq\xrightarrow{\lambda_{inc}} \qq'
$ for these states and layer.
On the other hand, the algorithm will not add the transition
$[\code{ctr=0}]\xrightarrow{\lambda_{dec}}[\code{ctr=0}]$ because the write path in $\lambda_{dec}$ is not enabled from $[\code{ctr=0}]$.

% Do one transition. layer is added because assertion is voilated:
% use earlier support example.
%assume(ctr not 0) [k in support] assert(not (ctr not 0))
%
%layer (\code{ctr=0})[decr-cas/true](*) not added because decr is not enabled from \code{ctr=0}

\end{example}


%\subsection{Proof of Thm.~\ref{thm:aut_layer_serialized}}
%\label{apx:aut_layer_serialized}
%
%\red{update}
We now discuss the correctness of this algorithm, i.e., the fact that it computes an SWO expression which is an abstraction of a quotient. We consider as quotient the set of traces defined as sequences of layer expression interpretations. Given a trace $\tr$ from this quotient, which is the trace of some execution $\exec$, every configuration  $C$ in $\exec$ where an interpretation of a layer $\lyr$ starts satisfies an automaton state $q$ with an outgoing transition labeled with $\lyr$ in the following sense: if $\lyr$ is a local layer, then the shared state in $C$ and the inputs of any invocation performing an iteration in that interpretation satisfy $q$, and if $\lyr$ is a write layer, then the shared state in $C$ and the inputs of any pair of invocations that perform an iteration following a read path in $\lyr$ and the write path in $\lyr$ satisfy $q$. This is a consequence of the fact that automaton states are obtained from pre-conditions of layer supports assuming the postcondition $\mathit{true}$. Then, for every interpretation of a layer $\lyr$ in $\exec$ going from a configuration $C$ to another configuration $C'$, there must exist an automaton transition labeled with $\lyr$ starting in a state $q$ satisfied by $C$ to a state $q'$ satisfied by $C'$. Although the condition used to add transitions in Algorithm~\ref{alg:alg} checks for feasibility of a restriction of the layer interpretation to a single iteration following a local path, local actions do not affect enabled-ness of actions executing in parallel, and therefore, that local path can be ``replicated'' to unboundedly-many copies.

==> hwq.tex <==
% !TEX root = paper.tex


%\newcommand{\enqinc}{\code{i:=back++}}
%\newcommand{\enqwr}{\code{items[i] = v}}
\newcommand{\enqinc}{\code{enqI}}
\newcommand{\enqwr}{\code{enqW}}
\newcommand{\deqT}{\code{deqT}}
\newcommand{\deqF}{\code{deqF}}
\newcommand\ttback{\code{back}}

\subsection{The Herlihy-Wing Queue.}
\label{sec:hwq}

The quotients of some data structures cannot be represented using layer automata. The Herlihy-Wing Queue~\cite{DBLP:journals/toplas/HerlihyW90} is one such example and it is notorious for  linearization points that depend on the future and that \emph{can not} be associated to fixed statements, see e.g.~\cite{DBLP:conf/cav/SchellhornWD12}!
%
The queue is implemented as an array of slots for items, with a shared variable \code{back} that indicates the last possibly non-empty slot. An \code{enq} atomically reads and increments \code{back} and then later stores a value at that location. A \code{deq} repeatedly scans the array looking for the first non-empty slot in a doubly-nested loop.
%
We show that the Herlihy-Wing queue quotient can
be abstracted by an expression 
$\left( \deqF^*\cdot (\enqinc)^+ \cdot\enqwr^* \cdot \deqT^*\right)^*$, 
where $\deqF$ captures dequeue scans that need to restart,
$\deqT$ scans succeed, $\enqinc$ reads/increments \ttback{} and 
$\enqwr$ writes to the slot.
%
For lack of space, a detailed discussion about how this expression abstracts
the quotient is given in Apx.~\ref{apx:hwq}. Importantly, linearization points in executions represented by this expression are \emph{fixed}, drastically simplifying reasoning from the general case where they are non-fixed.







==> layerautomata.tex <==
% !TEX root = paper.tex

%\subsection{Automated layer discovery}
%\label{sec:automation}
\section{Layer Automata}
%\label{apx:layerautomata}






==> layersautomaton.tex <==
%!TEX root = paper.tex
\section{Layer Automata}
\label{sec:layersautomaton}


%\todo{Discuss incompleteness, e.g., computing weakest-precondition from true, and refer to Michael/Scott section for an example. Be sure to discuss it there (the advancer layer self-loop when the next is not null.}


%The automaton has no notion of initial (or final) state, but its semantics as a set of traces will implicitly require that 


%The arcs of an LA are labeled with layers.
%We write $\sem{\qq{}}$ when referring to the KAT semantics of a given node $\qq{}$ in the automaton although this is not strictly necessary because they are one and the same. Typically, we will think of a node $\qq$ as a conjunction of tests. For the MSQ example, one node is 
%$([Q.head = Q.tail]\kdot[Q.head.next = null])$.
%
%\begin{definition}[Semantics of a layers automaton]
%For automaton $\Aut$, we define the semantics
%$\sem{\Aut\times \env} \subseteq \mathcal{P}(\Akat)\times(\mathbb{N} \rightarrow \tids)$, to yield pairs of the form $(\pth,\textsf{tidm})$ where $\pth$ is a sequence of actions, and $\textsf{tidm}$ maps those actions to thread identifiers.
%A trace can thus be constructed from such a pair as:
%$
%\tr_\textsf{tidm}^{\pth} = 
%\textsf{mapi} \; (\lambda a\;i. \textsf{tidm}(i):a)\; \pth
%$ and, for shorthand, we refer to this construction as 
%simply $\tr\in\sem{\Aut \times \env}$.
%\end{definition}
%
%\red{fix above. env is $(\tid,m(\As),\overline{\mathit{Val}})$}





%\SetKwFunction{kwWP}{WP}
%\SetKwFunction{kwSP}{SP}
%\SetKwFunction{kwDistinguish}{Distinguishing}
%\SetKw{kwLet}{let}
%\SetKw{kwIn}{in}
%\begin{algorithm}
%\KwIn{Method paths $\Pths = (\kro_1\cdot \condwr{b_1}{a_1},\kro_2\cdot\condwr{b_2}{a_2},\ldots)$}
%\KwResult{Layer automaton $\mathfrak{A}$}
%
%\Begin{
%\tcp{Uses WPs of write operations to determine predicates to distinguish ADT states}
%$\bar{\varphi}_{pre}$ := $\emptyset$\;
%\ForEach{$\kbaw \in \Pths$}{
%   $\bar{\varphi}_{pre} \stackrel{\cup}{=} $ \kwWP($\kbaw$)
%}
%\kwLet $[p_0,\ldots,p_k]$ = \kwDistinguish($\bar{\varphi}_{pre}$) \kwIn\;
%\kwLet $\qq{} : \mathbb{B}^k$ \kwIn\;
%\kwLet  $\qq{}_0$ be the initial state \kwIn\;
%\kwLet  readLoops : $\qq{} \rightarrow \mathcal{K}$ = ($\lambda \qq{}. 1$) \kwIn\;
%\tcp{Consider each method, each possible write path, from any possible $\qq{}$}
%\ForEach{$\kbaw \in \Pths$}{ 
%\ForEach{ $\qq{} \in \QQ{}$}{ 
%\red{what if $a_w = ret$?}\;
%\If{$\sem{ \qq{} } \cdot \kro_w \kdot b_w \neq 0$}{
%   \tcp{The write is enabled from $\qq{}$. Create transition layers to $\qq{}'$s.}
%   $b_{sp}$ := \kwSP($\sem{ \qq{} } \kdot \kbaw$)\;
%   \ForEach{ $\mathfrak{q'} \in \qq{}$ s.t. $\sem{\qq{}'} \kdot b_{sp} \neq 0$}{ 
%%   \tcp{Create an arc (layer) in $\mathfrak{A}$, with this write and all those who accordingly restart}
%   \kwLet  readers := $\{ \kro_r \kdot \condwr{b_r}{a_r} \in \Pths
%\mid \exists I. (\kbaw \itl{I} \kro_r) \kdot \overline{b}_{r} = 0\}$ \kwIn\;
%%   restarters := $\{  (q_m^0, \pth_{ro}, q_2) \mid 
%%      \exists s_{wr}, q_1. 
%%   (q_m^0, \pth_{ro}, b, s_{wr}, q_1, q_2) \in \wrPath(M)
%%   \wedge 
%%     ( \sem{\qq{}'} \wedge sp \wedge b \Rightarrow \textsf{false}) \}$\;
%%     \red{or: conflict graph is cyclic}\;
%   $\mathfrak{D} \stackrel{\cup}{=} \qq{} \xrightarrow{
% \kbaw \odot readers \red{fix}
%}\qq{}'$\; 
%      }
% 
%}
%%{
%%   \tcp{The write is disabled from $\qq{}$. Include this failed writer in $\qq{}$ restarts}
%%   readLoops[$\qq{}$] := readLoops[$\qq{}$] + $\pth_w^{ro}$\; 
%%}
%}
%}
%\tcp{Collect all the $\qq{} \rightarrow \qq{}$ layers, which don't change the ADT state}
%\ForEach{ $\qq{} \in \QQ{}$}{
%restarters := 1\;
%\ForEach{ $\kbaw\in \Pths$ }{
%   \If{$\sem{\qq{}} \kdot \kro_w \kdot b_w = 0$}{
%       restarters := restarters + $(\kro_w \kdot \overline{b}_w )$
%   }
%
%}
%$\mathfrak{D} \stackrel{\cup}{=} \qq{} \xrightarrow{restarters}\qq{}$\; 
%}
%\Return{$\mathfrak{A}=\langle \qq{}, \qq{}_0, K, \mathfrak{D} \rangle$}\;
%\red{draw automaton for MSQ and put in overview}\;
%\red{make counter.c}. \red{then array map}\;
%\red{ownership pointer}\;
%
%
%%Algorithm:
%%• forall ($pi_{pre},Cond,s\_{wr}$) in CFG
%%• compute pre-conditions sequentially.
%%• predicates P. 
%%• create automaton state for each valuation of precondition propositions
%%• find the arcs- compute the SP of a write path from each automaton state, to create an arc (q,q’)
%%   Check whether conjunction with q’ predicates is not false
%%• find all the *failing* restarts- what could be invalidated by the arc’s write.
%%   (Conflict graph is cyclic: read something that’s then written, then Cond-induced restart.)
%%   These go into the same layer.
%%• After a write, set R of immediate
%}
%%where $\wrPath(M)$ returns tuples
%%$(q_m^0, \pth_{ro}, b, s_{wr}, q_1, q_2)$
%%consisting of the read-only path $\pth_{ro}$ from a method entry $q_m^0$ up to automaton state $q$ having the pair of arcs 
%%$
%%q \xrightarrow{ \texttt{assume}(b); s_{wr} } q_1
%%$
%%and 
%%$
%%q \xrightarrow{ \texttt{assume}(\neg b)} q_2
%%$ corresponding, respectively, to the successful
%%conditional writing and the unsuccessful restart, looping back to $q_2$.
%\caption{\label{alg:alg} Constructing a layers automaton.}
%\end{algorithm}




%\vfill
%\pagebreak
%\paragraph{Examples}
%Here is a path from the MSQ: 
%\[\{true\} read(Qtail) \cdot read(Qtail.tl) \cdot assume(Qtail'=Qtail) \cdot  assume(isNull(next)) \cdot \{ tail.tl=next \} tail.tl=node\]


%\begin{theorem}[Soundness]
%Let $\QQ$ be the result of Algorithm~\ref{alg:alg}.
%For all $\tr\in\sem{\mathfrak{A}\otimes\env}$, there exists $\tr'\in \red{\sem{M\otimes\env}}$ such that $\tr\teq\tr'$.
%\end{theorem}
%
%
%\begin{theorem}[Completeness]
%Let $\QQ$ be the result of Algorithm~\ref{alg:alg}.
%For all $\tr\in \red{\sem{M\otimes\env}}$, there exists $\tr'\in\sem{\mathfrak{A}\otimes\env}$ such that $\tr\teq\tr'$.
%\end{theorem}


==> logs.tex <==
\section{Cion Output}
\tiny
\subsection{Descriptor}

\begin{verbatim}
 + begin Algorithm
checking if write(disclaim{l == lock | lock = myTid___0;}) is enabled from q:(lock == 0 && descriptor == 0) ... 
NOT enabled
checking if write(claim{l == lock | lock = myTid;}) is enabled from q:(lock == 0 && descriptor == 0) ... 
enabled
Trying layer: q(lock == 0 && descriptor == 0)--claim{l == lock | lock = myTid;}-->q(lock == 0 && descriptor == 0):  writePost is NOT feasible.
Trying layer: q(lock == 0 && descriptor == 0)--claim{l == lock | lock = myTid;}-->q(lock == 0 && ! (descriptor == 0)):  writePost is feasible.
>>> LAYER CREATED: q(lock == 0 && descriptor == 0)--claim{l == lock | lock = myTid;}-->q(lock == 0 && ! (descriptor == 0)) with the following readers:
 * reader(disclaim{last stmt: assume(! ((unsigned long )descriptor != (unsigned long )((struct node_t *)0)));}), interleaved at 0, see out/feas_5.c
  - did not find any feasible interleavings for reader(disclaim{last stmt: assume(! (l == 0));})
  - did not find any feasible interleavings for reader(disclaim{last stmt: _endARWfail_ = 1;})
 * reader(claim{last stmt: assume(! ((unsigned long )descriptor == (unsigned long )((struct node_t *)0)));}), interleaved at 0, see out/feas_16.c
  - did not find any feasible interleavings for reader(claim{last stmt: assume(! (l == 0));})
  - did not find any feasible interleavings for reader(claim{last stmt: _endARWfail_ = 1;})
  -> total there were 2 readers (out of 6) invalidated by the writer
Trying layer: q(lock == 0 && descriptor == 0)--claim{l == lock | lock = myTid;}-->q(! (lock == 0) && descriptor == 0):  writePost is NOT feasible.
Trying layer: q(lock == 0 && descriptor == 0)--claim{l == lock | lock = myTid;}-->q(! (lock == 0) && ! (descriptor == 0)):  writePost is NOT feasible.
checking if write(disclaim{l == lock | lock = myTid___0;}) is enabled from q:(lock == 0 && ! (descriptor == 0)) ... 
enabled
Trying layer: q(lock == 0 && ! (descriptor == 0))--disclaim{l == lock | lock = myTid___0;}-->q(lock == 0 && ! (descriptor == 0)):  writePost is NOT feasible.
Trying layer: q(lock == 0 && ! (descriptor == 0))--disclaim{l == lock | lock = myTid___0;}-->q(lock == 0 && descriptor == 0):  writePost is feasible.
>>> LAYER CREATED: q(lock == 0 && ! (descriptor == 0))--disclaim{l == lock | lock = myTid___0;}-->q(lock == 0 && descriptor == 0) with the following readers:
 * reader(disclaim{last stmt: assume(! ((unsigned long )descriptor != (unsigned long )((struct node_t *)0)));}), interleaved at 0, see out/feas_32.c
  - did not find any feasible interleavings for reader(disclaim{last stmt: assume(! (l == 0));})
  - did not find any feasible interleavings for reader(disclaim{last stmt: _endARWfail_ = 1;})
  - did not find any feasible interleavings for reader(claim{last stmt: assume(! ((unsigned long )descriptor == (unsigned long )((struct node_t *)0)));})
  - did not find any feasible interleavings for reader(claim{last stmt: assume(! (l == 0));})
  - did not find any feasible interleavings for reader(claim{last stmt: _endARWfail_ = 1;})
  -> total there were 1 readers (out of 6) invalidated by the writer
Trying layer: q(lock == 0 && ! (descriptor == 0))--disclaim{l == lock | lock = myTid___0;}-->q(! (lock == 0) && descriptor == 0):  writePost is NOT feasible.
Trying layer: q(lock == 0 && ! (descriptor == 0))--disclaim{l == lock | lock = myTid___0;}-->q(! (lock == 0) && ! (descriptor == 0)):  writePost is NOT feasible.
checking if write(claim{l == lock | lock = myTid;}) is enabled from q:(lock == 0 && ! (descriptor == 0)) ... 
NOT enabled
checking if write(disclaim{l == lock | lock = myTid___0;}) is enabled from q:(! (lock == 0) && descriptor == 0) ... 
NOT enabled
checking if write(claim{l == lock | lock = myTid;}) is enabled from q:(! (lock == 0) && descriptor == 0) ... 
NOT enabled
checking if write(disclaim{l == lock | lock = myTid___0;}) is enabled from q:(! (lock == 0) && ! (descriptor == 0)) ... 
NOT enabled
checking if write(claim{l == lock | lock = myTid;}) is enabled from q:(! (lock == 0) && ! (descriptor == 0)) ... 
NOT enabled
+ complete.
                (filename)    (states) (layers) (s) (queries)
RESULT: \texttt{bench/descriptor.c  } &   4 &   2 &  97.7ms &  61
\end{verbatim}

\subsection{Michael/Scott Queue}
\tiny
\begin{verbatim}
see logs/msq.tex
\end{verbatim}

==> msqlayers.tex <==
% !TEX root = paper.tex


